Testing lowered isothermal models with direct N-body simulations of globular clusters

Several self-consistent models have been proposed, aiming at describing the phase space distribution of stars in globular clusters. This study explores the ability of the recently proposed LIMEPY models (Gieles & Zocchi) to reproduce the dynamical properties of direct N-body models of a cluster in a tidal field, during its entire evolution. These dynamical models include prescriptions for the truncation and the degree of radially-biased anisotropy contained in the system, allowing us to explore the interplay between the role of anisotropy and tides in various stages of the life of star clusters. We show that the amount of anisotropy in an initially tidally underfilling cluster increases in the pre-collapse phase, and then decreases with time, due to the effect of the external tidal field on its spatial truncation. This is reflected in the correspondent model parameters, and the best-fit models reproduce the main properties of the cluster at all stages of its evolution, except for the phases immediately preceding and following core collapse. We also notice that the best-fit LIMEPY models are significantly different from isotropic King models, especially in the first part of the evolution of the cluster. Our results put limits on the amount of radial anisotropy that can be expected for clusters evolving in a tidal field, which is important to understand other factors that could give rise to similar observational signatures, such as the presence of an intermediate-mass black hole.

==> newcommands.tex <==

\def\limepy{\texttt{\small{LIMEPY}}}
\def\scipy{\texttt{\small{SCIPY}}}
\def\numpy{\texttt{\small{NUMPY}}}
\def\matplotlib{\texttt{\small{MATPLOTLIB}}}
\def\python{\texttt{\small{PYTHON}}}
\def\integrate{\texttt{\small{INTEGRATE}}}

\def\intfrac[#1,#2]{I_{#1}^{#2}}
\def\derfrac[#1,#2]{D_{#1}^{#2}}

\newcommand{\rvec}{\textbf{\emph{r}}}
\newcommand{\vvec}{\textbf{\emph{v}}}
\newcommand{\Jvec}{\textbf{\emph{J}}}

\newcommand{\fone}{\tfrac{1}{2}}
\newcommand{\fthree}{\tfrac{3}{2}}
\newcommand{\ffive}{\tfrac{5}{2}}
\newcommand{\fseven}{\tfrac{7}{2}}

\newcommand{\gfone}{g+\tfrac{1}{2}}
\def\dhalf{D^{1/2}}
\def\jhalf{J^{1/2}}

\def\ahat{\hat{A}}
\def\dr{{\rm d}}
\def\dawsn{F}
\def\hyp{{_1}F_1}
\def\E{\mathcal{E}}
\def\erf{{\rm erf}}
\def\ehat{\hat{E}}
\def\erfi{{\rm erfi}}
\def\dfk{f_{\rm K}}
\def\dfm{f_{\rm M}}
\def\dfw{f_{\rm W}}
\def\fnu{f^{(\nu)}}
\def\jhat{\hat{J}}
\def\jmax{J_{\rm max}^2}



\def\Eg{E_\gamma}
\def\Etot{E_{\rm tot}}
\def\gdos{\mathpzc{g}}
\def\Ncomp{N_{\rm comp}}

\def\onehalf{\textstyle{\frac{1}{2}}\displaystyle}
\def\threehalf{\textstyle{\frac{3}{2}}\displaystyle}
\def\fivehalf{\textstyle{\frac{5}{2}}\displaystyle}
\def\sevenhalf{\textstyle{\frac{7}{2}}\displaystyle}
\def\ninehalf{\textstyle{\frac{9}{2}}\displaystyle}

\def\gone{g+\onehalf}
\def\gthree{g+\threehalf}
\def\gfive{g+\fivehalf}
\def\henon{H\'{e}non}

\def\kms{{\rm km}\,{\rm s}^{-1}}

\def\rmm{r_{\rm m}}
\def\rh{r_{\rm h}}
\def\rhhat{\hat{r}_{\rm h}}
\def\rhat{\hat{r}}
\def\rrahat{\hat{p}}
\def\rahat{\hat{r}_{\rm a}}
\def\rajhat{\hat{r}_{{\rm a},j}}
\def\rv{r_{\rm v}}
\def\rvhat{\hat{r}_{\rm v}}
\def\rking{r_{\rm s}}
\def\ra{r_{\rm a}}
\def\rs{r_{\rm s}}
\def\ms{M_{\rm s}}
\def\rt{r_{\rm t}}
\def\rj{r_{\rm J}}
\def\rthat{\hat{r}_{\rm t}}
\def\pc{{\rm pc}}
\def\phit{\phit_{\rm t}}
\def\phat{\hat{p}}
\def\phihat{\hat{\phi}}
\def\rhohat{\hat{\rho}}
\def\rhoint{\mathcal{I}^{\rho}}
\def\fintone{\mathcal{I}_{F,1}}
\def\finttwo{\mathcal{I}_{F,2}}
\def\rhointnull{\mathcal{I}_0^{\rho}}
%\def\vsqint{\mathcal{I}^{\rho{v}^2}}
\def\vsqint{\mathcal{I}^{\rho \sigma^2}}
\def\vrsqint{\mathcal{I}^{\rho \sigma_{\rm r}^2}}
\def\vtsqint{\mathcal{I}^{\rho \sigma_{\rm t}^2}}
%\def\vtsqint{\mathcal{I}^{\rho{v}_{\rm r}^2}}
%\def\vtsqint{\mathcal{I}^{\rho{v}_{\rm t}^2}}
%\def\mvsq{\langle {v}^2\rangle}
\def\mvsq{\sigma^2}
\def\sigmaoned{\sigma_{\rm 1d}}
\def\sigmaonedj{\sigma_{{\rm 1d}, j0}}
\def\sigmahat{\hat{\sigma}}
\def\sigmathat{\hat{\sigma}_{\rm t}}
\def\sigmarhat{\hat{\sigma}_{\rm r}}
\def\sigmat{\sigma_{\rm t}}
\def\sigmar{\sigma_{\rm r}}
\def\sigmatheta{\sigma_\theta}
\def\sigmaphi{\sigma_\varphi}
\def\mvhatsq{\langle \hat{v}^2\rangle}
\def\rvec{\textbf{\emph{r}}}
\def\vvec{\textbf{\emph{v}}}
\def\xvec{\textbf{\emph{x}}}
\def\mhat{\hat{M}}
\def\Uhat{\hat{U}}
\def\uhat{\hat{u}}
\def\vesc{v_{\rm esc}}
\def\vhat{\hat{v}^2}
\def\ut{u_{\rm t}}
\def\ur{u_{\rm r}}
\def\vrhat{\hat{v}_{\rm r}^2}
\def\vthat{\hat{v}_{\rm t}^2}
\def\khat{\hat{k}}
\def\vr{v_{\rm r}}
\def\vt{v_{\rm t}}
\def\vtheta{v_\theta}
\def\vphi{v_\varphi}
\def\vrms{v_{\rm rms}}
\def\vrmsr{\langle v_{\rm r}^2 \rangle}
\def\vrmst{\langle v_{\rm t}^2 \rangle}
\def\vrmsj{v_{{\rm rms},j}}
\def\vhatrmsj{\langle \hat{v}_{j}^2\rangle^{1/2}}
\def\vrmsjnot{\langle {v}_{j,0}^2\rangle^{1/2}}

\def\msun{\mbox{M}_{\rm \odot}}


